RT-DBSCAN: Accelerating DBSCAN using Ray Tracing Hardware

General Purpose computing on Graphical Processing Units (GPGPU) has resulted in unprecedented levels of speedup over its CPU counterparts, allowing programmers to harness the computational power of GPU shader cores to accelerate other computing applications. But this style of acceleration is best suited for regular computations (e.g., linear algebra). Recent GPUs feature new Ray Tracing (RT) cores that instead speed up the irregular process of ray tracing using Bounding Volume Hierarchies. While these cores seem limited in functionality, they can be used to accelerate n-body problems by leveraging RT cores to accelerate the required distance computations. In this work, we propose RT-DBSCAN, the first RT-accelerated DBSCAN implementation. We use RT cores to accelerate Density-Based Clustering of Applications with Noise (DBSCAN) by translating fixed-radius nearest neighbor queries to ray tracing queries. We show that leveraging the RT hardware results in speedups between 1.3x to 4x over current state-of-the-art, GPU-based DBSCAN implementations.

==> temp.tex <==


\author{\IEEEauthorblockN{Vani Nagarajan}
\IEEEauthorblockA{\textit{Electrical and Computer Engineering} \\
\textit{Purdue University}\\
West Lafayette, USA \\
nagara16@purdue.edu}
\and
\IEEEauthorblockN{Milind Kulkarni}
\IEEEauthorblockA{\textit{Electrical and Computer Engineering} \\
\textit{Purdue University}\\
West Lafayette, USA \\
milind@purdue.edu}
}

%Eval Fig 7
\begin{subfigure}[b]{0.43\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/3diono-scalable-num-intersections.pdf}
         \caption{Impact of dataset size on number of intersections}
         \label{fig:num-intersections}
     \end{subfigure}
     \caption{Scalability of results}
     \label{fig:scalability}

     II B 2):The Optix API \cite{prog-guide} provides programmable kernels (programs) to accelerate ray tracing applications by leveraging the RT cores in GPUs. These programs allow the user to write customize shader programs.

%ref.bib
@article{Evangelou2021RadiusSearch,
  author =       {I. Evangelou and G. Papaioannou and K. Vardis and A. A. Vasilakis}, 
  title =        {Fast Radius Search Exploiting Ray Tracing Frameworks},
  year =         2021,
  month =        {February},
  day =          5,
  journal =      {Journal of Computer Graphics Techniques (JCGT)},
  volume =       10,
  number =       1,
  pages =        {25--48},
  url =          {http://jcgt.org/published/0010/01/02/},
  issn =         {2331-7418}
} 

@inproceedings {wald19,
booktitle = {High-Performance Graphics - Short Papers},
editor = {Steinberger, Markus and Foley, Tim},
title = {{RTX Beyond Ray Tracing: Exploring the Use of Hardware Ray Tracing Cores for Tet-Mesh Point Location}},
author = {Wald, Ingo and Usher, Will and Morrical, Nathan and Lediaev, Laura and Pascucci, Valerio},
year = {2019},
publisher = {The Eurographics Association},
ISSN = {2079-8687},
ISBN = {978-3-03868-092-5},
DOI = {10.2312/hpg.20191189}
}

%NGSIM fig
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[scale=0.5]{figures/eps-ngsim.pdf}
         \vspace{-0.5em}
         \caption{Speedup on varying search radius ($\varepsilon$)}
         \label{fig:ngsim_eps}
     \end{subfigure}    
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[scale=0.5]{figures/datasize-ngsim.pdf}
         \vspace{-0.5em}
         \caption{Speedup on varying dataset size}
         \label{fig:ngsim_ds}
     \end{subfigure}
     \caption{Speedup over FDBSCAN on varying $\varepsilon$ and dataset size for NGSIM}
     \label{fig:ngsim}
     \vspace{-0.5em}
\end{figure*}

%NGSIM Table
\begin{table}[h]
%\centering
    \begin{tabular}{|c| c| c| c|} 
    \hline
       \textbf{Dataset size } & \textbf{FDBSCAN(s)} & \textbf{RT-DBSCAN(s)} & \textbf{Speedup} \\
       \hline
       500K & 12.7 & 0.03 & 423.33\\
       \hline
       1M & 72.8 & 0.06 & 1213.33 \\
       \hline
       2M & 364.6  & 0.13 & 2804.61\\
       \hline
       4M & 1631.4 & 0.3 & 5438\\
       \hline
       8M & 6964.1 & 1.26 & 5527.06\\
       \hline
   \end{tabular}
   \caption{Execution time (in seconds) for NGSIM dataset on varying dataset size}
    \label{table:ngsim-dataset-size}
     \vspace{-1.5em}
\end{table}

\begin{table}[h]
%\centering
    \begin{tabular}{|c| c| c| c|} 
    \hline
    \textbf{Search radius ($\varepsilon$) } & \textbf{FDBSCAN(s)} & \textbf{RT-DBSCAN(s)} & \textbf{Speedup} \\         
       \hline
        0.0001 & 64.72 & 0.0257 & 2518.28\\
       \hline
        0.00025 & 64.77 & 0.0259 & 2500.77\\
       \hline
        0.0005 & 64.74 & 0.0259 & 2499.61\\
       \hline
        0.00075 & 64.71 & 0.026 & 2488.84\\
       \hline
       0.001 & 64.74 & 0.0259 & 2499.61\\
       \hline
   \end{tabular}
   \caption{Execution time (in seconds) for NGSIM dataset on varying search radius ($\varepsilon$)}
    \label{table:ngsim-eps}
     \vspace{-1.5em}
\end{table}

%BVH image
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/bvh_img.png}
    \caption{(a) 2D rectangular bounding boxes for the objects and intermediate bounding volumes (b) Bounding Volume Hierarchy built from the bounding boxes in (a)}
    \label{fig:bvh_img}
    \vspace{-1.6em}
\end{figure}
